Autonomous Aerial Robot for High-Speed Search and Intercept Applications

In recent years, high-speed navigation and environment interaction in the context of aerial robotics has become a field of interest for several academic and industrial research studies. In particular, Search and Intercept (SaI) applications for aerial robots pose a compelling research area due to their potential usability in several environments. Nevertheless, SaI tasks involve a challenging development regarding sensory weight, on-board computation resources, actuation design and algorithms for perception and control, among others. In this work, a fully-autonomous aerial robot for high-speed object grasping has been proposed. As an additional sub-task, our system is able to autonomously pierce balloons located in poles close to the surface. Our first contribution is the design of the aerial robot at an actuation and sensory level consisting of a novel gripper design with additional sensors enabling the robot to grasp objects at high speeds. The second contribution is a complete software framework consisting of perception, state estimation, motion planning, motion control and mission control in order to rapid- and robustly perform the autonomous grasping mission. Our approach has been validated in a challenging international competition and has shown outstanding results, being able to autonomously search, follow and grasp a moving object at 6 m/s in an outdoor environment

==> upo.tex <==
The main objective of Challenge 3 is to autonomously extinguish a series of simulated fires in an urban high rise building firefighting scenario. In particular, a team of robots has to extinguish a set of fires using water, including fires inside the building and located in its facade. Furthermore, fires located at ground level outside the building must be extinguished using fire blankets carried by the robots.

To accomplish the mission, we use a team of up to 3 UAVs and 1 UGV. In the following, we describe the proposed robotic team and their main modules. Then, we describe the cooperation in the team.  

\subsection{The robot team}

\subsubsection{Unmanned ground vehicle}
% David, review
The ground platform used for Challenge 3 is a 6-wheeled robot with independent traction system and a pan\&tilt mechanism on top. The robot is able to navigate at a maximum speed of 0.7 m/s and it has battery autonomy for more than 4 hours of operation (motion and sensing/computation). The robot integrates an i7 computer, local sensing and a 3D LIDAR. The hardware used in the ground platform is (see Fig. \ref{fig:siar_sensors}):
\begin{itemize}
    \item Onboard computer: 5NUC5i7RYB.
    \item GPS sensor UBlox 8.
    \item IMU: ArduIMUv3.
    \item Infrared camera: A compact SeekThermal camera mounted on a pan\&tilt mechanism on top of the robot. The images are used for fire detection.
    \item 3D LIDAR: A 3D OS-1-16 LIDAR manufactured by Ouster has been installed on top of the robot. The information gathered by this sensor is used for localization and mapping.
    \item 2D LIDAR: A Hokuyo UTM-30LX sensor is installed. The information of this sensor is used for local obstacle detection/avoidance.
    \item Orbbec ASTRA camera. Used for providing the operator with images to allow remotely operating the platform. It is also used for indoor local obstacle avoidance.
\end{itemize}

\begin{figure}[h]
	\centering
    \includegraphics[width = 0.47\textwidth]{images/siar_sensors_1.jpeg}
    \includegraphics[width = 0.47\textwidth]{images/siar_sensors_2.jpeg}
	\caption{Ground platform used for Challenge 3.}
	\label{fig:siar_sensors}
\end{figure}

\subsubsection{Unmanned aerial vehicles}
Regarding to the aerial platforms, the aerial robot models used for the competition will be adaptations of the DJI Matrice 210 V2 and the DJI Matrice 600 Pro. The aerial platforms are also equipped with a OS-1-16 LIDAR manufactured by Ouster, installed to the bottom of the robots. The LIDAR is able to provide 320k 3D points per second, ranging from 0.2 to 120 meters. The purpose of this sensor is threefold:
\begin{itemize}
    \item Environment mapping and odometry. This sensor is the basis for the generation of the 3D map of the environment. It is also used to compute an accurate robot odometry in the UAVs. 
    \item Robot localization. The 3D LIDAR is used as main sensor for robot localization in all robots, UAVs and UGV.
    \item Obstacle detection for robot navigation. The robot local planner uses this information to detect mid/long range obstacles (more than 2 meters) in order to properly react on time.
\end{itemize}

Fig. \ref{fig:m600} shows the DJI Matrice 600 Pro used for the preliminary experiments.

\begin{figure}[h]
	\centering
    \includegraphics[width = 0.42\textwidth]{images/M600.jpeg}
    \includegraphics[width = 0.45\textwidth]{images/m600-building.jpg}
	\caption{DJI Matrice 600: one of the aerial platforms used for Challenge 3.}
	\label{fig:m600}
\end{figure}

\subsection{3D Mapping and Localization}
One of the main issues in Challenge 3 is the localization of the robots. They should localize seamlessly and accurately in GPS and GPS-denied environment (inside the building), with a smooth transition among them. 

The mapping and localization system proposed consists of two main modules (see Fig. \ref{fig:map_localization}): a LIDAR-based odometry and an online map-based global localization module. These systems update the global map during the mapping phase, and estimates the global position of the robot into the map during the mission. Next sections describe each module of the implemented system. While there are differences in the UAV and UGV, both are based on the same principles.

% Figure Mapping and localization system
\begin{figure}[!tb]
	\centering
    \includegraphics[scale = 0.35]{images/map_localization.jpeg}
	\caption{Mapping and localization system implemented in the all the platforms.}
	\label{fig:map_localization}
\end{figure}

\subsubsection{3D Mapping and multi-sensor odometry}
The base for the mapping and localization systems is an odometry system that allows to estimate the relative motion of the robot. The LIDAR-based odometry module considers IMU and 3D LIDAR in order to compute a reliable 6DoF robot odometry in the environment. This module provides short-term aligned scans that can be used for local mapping and a map of the environment. It integrates the IMU estimation together with a LIDAR-based mapping process to provide global consistency to the mapping process.

The LIDAR-based odometry module implements an advanced LOAM system \cite{LOAM}, which decomposes the original problem into scan registration and mapping. The first problem is solved as online motion estimation. The second one conducts mapping as batch optimization (similar to iterative closest point, ICP \cite{ICP}). The system computes high-precision motion estimates and maps. Therefore, the accuracy of the localization of the robot and of the map is considerably improved.

The system implemented fuses the information from 3D LIDAR and IMU data. Some modifications have been implemented with respect to the original LOAM system \cite{LOAM}. The original one uses the point cloud from a 2D LIDAR sensor. In our implementation, the first motion estimation is computed from 3D point cloud and acceleration values from IMU sensor. 

During the mapping stage, other sensors as GPS are also recorded. This information is later on used to compute the relative transformation between the computed 3D map and the GPS coordinate system for multi-sensor localization.

\begin{figure}[!tb]
	\centering
    \includegraphics[width = 0.45\textwidth]{images/map_guillena}
	\caption{Example of 3D map computed outdoors with data provided by one robot.}
	\label{fig:map_example}
\end{figure}

%This estimation is computed by using a non-linear optimizer based on Ceres solver library. This library reduces the computational load and complexity with respect to previous implementations of the LOAM system.
%The motion model considered allows us to linear interpolate the pose transform within a sweep for the points that are received at different times. Let $t$ be the current timestamp, and recall that $t_{k+1}$ is the starting time of sweep $k+1$.
%Regarding the LIDAR odometry algorithm used, the inputs are the 3D point cloud from the last sweep, $P_k$, the growing 3D point cloud of the current sweep, $P_{k+1}$, the pose transformation from the last recursion, $T^{L}_{k+1}$, and current values of roll and pitch from acceleration values of IMU sensor. If a new sweep is started, $T^{L}_{k+1}$, is set to zero. Then, the algorithm extracts feature points from $P_{k+1}$ using roll and pitch values from IMU sensor, to construct $E_{k+1}$ and $H_{k+1}$, which are the sets of edge points and planar points extracted respectively. For each feature point, we find its correspondence in $P_k$. The distance between feature points and its correspondence is considered to assign weights. Once the weights are assigned, a nonlinear function has to be solved:

%EQ1

%where each row of $f$ corresponds to a feature point and $d$ is the corresponding distance.

%Then, the Jacobian matrix of $f$ with respect to $T^{L}_{k+1}$ is computed, denoted as $J$, where $J = \delta f/\delta T^{L}_{k+1}$. Thus, (1) can be solved through nonlinear iterations by minimizing d toward zero:

%EQ2

%where $J$ is the Jacobian matrix and \lambda is determined by the Levenberg-Marquardt algorithm.

%The nonlinear optimization terminates if convergence is found, or the maximum iteration number is met. The $P_{k+1}$ is reprojected to timestamp tk+2 when the algorithm reaches the end of a sweep and the estimated motion during the sweep is estimated.

\subsubsection{Multi-sensor robot localization}

Once the map is generated, another module is in charge of localizing the robot within the map built during the execution of the different missions. This module provides a robust global position of the robot in the map. The algorithm is based on Monte Carlo localization (MCL) approach and extends previous author work presented in \cite{Perezgrau17Iros}.

The starting point of the algorithm is an initial belief of the robot pose probability distribution, which determines the distribution of a set of position hypotheses around such pose. We call these hypotheses particles, and they are propagated following the robot motion model each time its pose changes. Every time new sensor readings are received, each particle evaluates its accuracy by checking how likely it would receive such sensor reading at its current pose. The next step of the algorithm is redistributing (resampling) the particles to new poses that are more likely to be accurate. This is an iterative process that involves moving, sensing, and resampling, while all the particles should converge to a single cluster near the true pose of the robot.

One of the main benefits of the MCL approach is the reduced computation required. The approach only evaluates the sensors when the robot moves above some  given thresholds in both translation and rotation. When the robot moves above one or both thresholds, it launches one update cycle: predicting robot position according to odometry, updating position hypotheses based on sensors and re-sampling the hypotheses space when required. 

Thus, the particle filter consists of $N$ particles $p_i$, each one with the following state vector $p_{i}=[x, y, z, \Psi]_{t}$. where $\Psi$ refers to the yaw angle of the robot. Note how the robot roll and pitch angles are not included into the robot pose definition. These angles are available and accurate enough in the robot through the use of its onboard IMU. They are fully observable and their values are usually accurate. This greatly reduces the computational complexity of the algorithm, allowing for real-time onboard computation. Each particle has an associated weight $w_i$ such as $\Sigma_i^N(w_i)=1$. 

The particles are initialized by setting the initial position and distributing them in the hypotheses space. The information from the LIDAR-based odometry provides increments of the robot state vector and it is used to compute a priori distribution of the particles. Thus, considering that the robot is a non-holonomic systems, the state of the particles will evolve according to the following expressions for particle $i$:

\begin{equation}
    x^{t+1}_{i}=x^{t}_{i}+\Delta x \times \cos (\Psi^{t}_{i})-\Delta x \times \sin (\Psi^{t}_{i})
\end{equation}
\begin{equation}
    y^{t+1}_{i}=y^{t}_{i}+\Delta x \times \sin (\Psi^{t}_{i})-\Delta x \times \cos (\Psi^{t}_{i})
\end{equation}  
\begin{equation}
    z^{t+1}_{i}=z^{t}_{i}+\Delta z 
\end{equation}  
\begin{equation}
    \Psi^{t+1}_{i}=\Psi^{t}_{i}+\Delta \Psi
\end{equation}

The values of $\Delta x$, $\Delta y$, $\Delta z$, and $\Delta \Psi$ are drawn randomly following a normal distribution centered in their actual values and standard deviations proportional to each increment itself.

The following sensor reading are used to update the weight associated to each particles hypothese: The point clouds provided by the 3D LIDAR sensor, the 3D Position provided by the GPS, the robot roll, pitch and yaw provided by the IMU and the height above the ground provided by the altitude sensor.

These sensor are integrated into the MCL differently, according to the following criteria:
\begin{itemize}
    \item The point clouds are transformed to each particle pose in order to find correspondences between the cloud and what the map should look like from that particle’s pose. Since this is very expensive computationally, we first compute a 3D probability grid as in \cite{Hornung10}, in which each position stores a value of how likely it is that such position falls within an occupied point of the map, instead of storing binary information about occupancy as in the provided map. Each 3D position $p_i$ of the grid is then filled with probability values according to a specific Gaussian distribution centered in the closest occupied point in the map from $p_i$, $map_i$, and whose variance $\sigma^2$ depends on the sensor noise used in the approach.
    \begin{equation}
    grid(p_i) = \frac{1}{{ \sqrt {2\pi \sigma^2 } }} e^{{{ - ||p_i - map_i || ^2 } \mathord{\left/ {\vphantom {{ - ||p_i - map_i || ^2 } {2\sigma ^2 }}} \right. \kern-\nulldelimiterspace} {2\sigma ^2 }}}
    \end{equation}
    Such probability grid only needs to be computed once, it is not required to be updated for a given environment, and relieves from performing numerous distance computations between each cloud point for each particle and its closest occupied point in the map. Besides, each point cloud is first transformed according to the current roll and pitch provided by the on-board IMU. This transformation is done just once per update, reducing the computational requirements as well.
    Then, for every point of the transformed cloud, we access its corresponding value in the 3D probability grid. Such value would be an indicator of how likely is that point to be part of the map. By doing this with every point of the cloud and adding all the probability values, we obtain a figure of how well that particle fits the true location of the aerial robot according to the map.

    Finally, the weight $w_i$ of each particle $\mathbf{p}_i$ is computed. Assuming that the point cloud is composed of $M$ 3D points $\mathbf{c}_j$, the weight is computed by adding all the associated probability grid values as follows:
    \begin{equation}
    w_i^{map}=\frac{1}{M}\sum_{j=1}^{M}grid\mathbf(\mathbf{p}_i(\mathbf{c}_j))
    \end{equation}
    \noindent where $\mathbf{p}_i(\mathbf{c}_j)$ stands for the transformation of the point to the particle's state, and $grid(\mathbf{p}_i(\mathbf{c}_j))$ is the evaluation of the probability grid in such transformed position.
    
    \item The position measurements provided by the GPS are used to check how well each particle hypothesis matches the sensor reading. 
    First, the GPS position is transformed into a local metric estimation into the map. Then, a $w^{gps}$ is computed for each particle. Assuming a GPS measurement $\mathbf{x}^{gps}$, the associated weight $w_i^{gps}$ is is computed as follows:
    \begin{equation}
        w_i^{gps}=\frac{1}{{ \sqrt {2\pi \sigma^2 } }} e^{{{ - ||p_i - x^{gps} || ^2 } \mathord{\left/ {\vphantom {{ - ||p_i - x^{gps} || ^2 } {2\sigma ^2 }}} \right. \kern-\nulldelimiterspace} {2\sigma ^2 }}}
    \end{equation}
    \noindent Where the distance computation dismisses the altitude contribution of the GPS, which is subject to significant noise. Also, the standard deviation of the GPS measurement $\sigma$ is computed empirically to account for GPS errors in single configuration.
    
    \item The height above the ground is integrated into the MCL through the re-sampling stage. Instead of including the information as a regular update, we decided to include this information into the re-sampling, forcing the hypotheses to be distributed around the altitude provided by the robot altimeter. This way, we can reduce the dispersion of the particles around Z axis, which is easily observable by means of different sensors as laser altimeter, barometer or GPS altitude. 
    
    \item IMU yaw angle is also integrated through the re-sampling stage. The rationale behind this decision is also based on the computational optimization and the nature of the yaw angle. In the experiments area, the yaw angle is assumed to be slightly distorted by the environment, so that we can trust the estimation from the magnetometer. Thus, everytime a new re-sampling is performed, the orientation of the particles are drawn from a Gaussian distribution centered in the latest yaw value provided by the IMU.
    
\end{itemize}

Finally, GPS and point-cloud updates are integrated into the filter. Given the distinct nature of the two technologies involved, we calculate separate weights for each sensing modality. A weighted average is used to obtain the final weight of each particle:
\begin{equation}
w_i=\alpha*w_i^{map}+(1-\alpha)*w_i^{gps}
\label{eq:alpha}
\end{equation}
\noindent where $\alpha$ is chosen depending on the particularities of the indoor environment where the robot is going to operate. If the map used in the MCL does not contain the full environment or its accuracy is not enough to trust the map matching, $\alpha$ should be lower than $0.5$. Whereas if GPS measurements are not accurate, $\alpha$ should be higher. 

This approach is used for both robot systems, ground and aerial. However some parameters are different between both platforms:
\begin{itemize}
    \item The dispersion in Z axis is very small in the predictive model of the ground robot. This relates with the fact that the UGV moves in 2D.
    \item The UGV does not integrates height sensors, for the same reason.
    \item The yaw angle is not integrated into the UGV. 
\end{itemize}

 




\subsection{Autonomous robot navigation}

After having a reliable localization, tasks such as where to go, follow a path or reach a goal should be addressed. The proposed autonomous navigation system consists of global and local planner. It generates safe paths from two configurations of the robot. A 3D planner has been implemented in the aerial platforms and a 2D planner in the ground platform. The implemented planner for the MBZIRC competition is an extended version of the planner presented in \cite{Perezgrau18_3}.

The Global Planner computes a path from the global map. The inputs are the mission plan generated by the operator, the map of the environment and the robot localization given by the MCL approach. The output is a feasible and safe path that should be followed in order to fulfill the mission plan. 

The planner is based on a variation of the any-angle path planning Theta* called Lazy Theta* \cite{THETA}. An advantage of this algorithm is the optimization of the computational load. Other advantages of this graph-based algorithm with respect to sampling-based algorithms is that its result is closed the shortest path and its solution is always the same. Furthermore, it gets a very low computation time and a high repeatability. These characteristics make this algorithm suitable to address the tasks of the MBZIRC competition.

Fig. \ref{fig:theta} shows some of these advantages in a complex scenario where the solution is difficult to find. Note that Lazy Theta* algorithm computes quickly the shortest path.

\begin{figure}[t]
	\centering
   \includegraphics[scale = 0.35]{images/theta_star}
	\caption{Example of trajectory computed by the Lazy Theta* algorithm. Initial position (black square) is in the top and final position at the bottom of the image.}
	\label{fig:theta}
\end{figure}

Lazy Theta* algorithm digs into optimizations of Theta*, reducing the number of line-of-sight checks required and optimizing the algorithm. It is a variant of Theta* and thus it propagates information along graph edges (to achieve a short runtime) without constraining the paths to graph edges (to find "any-angle" paths). The algorithm is based on the A* algorithm, and this last one is basically the Dijkstra algorithm with Euclidean distance as heuristic. Theta* takes into account the line of sight between neighbours allowing any-angle paths, and finally Lazy Theta* reduces the line of sight checks improving computation times by keeping the same paths as Theta*.

On the other hand, the Local planner creates a plan locally dealing with dynamic obstacles thanks to the measurements obtained from the onboard 3D LIDAR. It is in charge of following the global path computed by the global planner and should also replan quickly a safe trajectory when an unexpected event takes place such as an unknown obstacle. It takes as input the global path generated by the global planner and the local map built by using the measurements of the onboard sensors in order to make the crawler executes the input path. As output, it provides a free-collision trajectory to the path tracker module.


\subsection{Fire perception and extinguishing}
In order to accomplish the mission, we need to detect fires and estimate their positions by using sensors on board the robots. 

\begin{figure}[t]
	\centering
    \includegraphics[scale = 0.5]{images/detection}
	\caption{Fire segmentation on the infrared images during an extinguishing action. From left to right it can be seen how the temperature decreases when applying water.}
	\label{fig:firedetection}
\end{figure}

\subsubsection{Fire segmentation}
%Fire segmentation
The main sensor related to fire perception is the miniature infrared thermal camera mentioned above. The camera can detect temperatures between -40º to 330º Celsius.

Fire detection is carried out by analyzing the infrared images provided by the cameras. A calibration procedure approximately transforms the raw data obtained by the cameras to temperature ranges. Then, given the clear difference of temperatures between the fire and the surroundings, a thresholding operation is performed to segment the fire pixels.

As a result, the fire detection module provides coordinates on the image plane of fire spots. Fig. \ref{fig:firedetection} shows an example of the results obtained in local tests considering the IR device used in the challenge to emulate the fire IR signature.


\subsubsection{Fire position estimation}

The fire segmentation results mentioned above will be used for the visual servoing final approach to extinguish the fire (see below). However, during the exploration of the scenario we need to estimate the 3D position of the fire spots to plan the approximation goals for fire extinguishing.

\begin{figure}[t]
	\centering
    \includegraphics[scale = 0.5]{images/firePositionFinal}
	\caption{Information from the camera pose and LIDAR is fused in time to estimate the position of the fire.}
	\label{fig:fireposition}
\end{figure}

From the fire position in pixel coordinates it is not possible to the estimate the 3D position of the fires, as there is no information about the range to the fires. In order to obtain the range, the LIDAR information is considered. The LIDAR values are mapped to the image coordinates and associated to the fire object, so that a range can be estimated. This is not always possible given the resolution of the LIDAR (and depending on the actual distance to the fire). In that case, the range is estimated considering the maximum distances according to the 3D map of the environment. Each measurement is associated with a covariance matrix that reflects the uncertainty on the range, which is adapted according to the estimated range (in the latter case, a large uncertainty is associated to the range), and other aspects like the position of the robot.  

Then, an Information Filter is used to fuse in time the measurements about the position of the fire from different view points in order to triangulate the fire position, as in \cite{triangicra15}. Fig. \ref{fig:fireposition} shows the estimated position of a fire and the associated uncertainty in a mission inside a building. This filter allows to consider also measurements from multiple robots for the triangulation procedure.



\subsubsection{Fire extinguishing}
%Fire extinguishing hardware and control
The fire position estimation can be used to approach the fire sources from an adequate vantage point. Once the robot is located at a attacking distance to the fire, a fire extinguishing task can be launched. This consists on aiming adequately the extinguishing device, checking the presence of the fire and releasing the water, for the fires in the building. 


%The hardware used is (see Fig. \ref{fig:extinguishing_siar_drone}):
%\begin{itemize}
%    \item Arduino Uno
%    \item 2 Mini Water Pump 5V, 4.8 W, 300 cm elevation
%    \item MOSFET switching module controlled by Arduino Uno
%    \item Silicone tube 7x10 mm
%\end{itemize}

\begin{figure}[t]
	\centering
    \includegraphics[scale = 0.35]{images/extinguishing_siar_drone.jpg}
	\caption{Fire extinguishing systems installed on ground platform (left) and a DJI Matrice M210 v2 (right).}
	\label{fig:extinguishing_siar_drone}
\end{figure}

%The extinguishing system uses the Arduino Uno board to communicate with the robot PC through the serial port. Thus, from ROS we can manage send messages to Arduino, wich it the responsible to activated or deactivated the water pumps to turn off the fire. The serial communication between Arduino and PC is possible using the rosserial package. Fig. \ref{fig:diagram_extinguishing_drone} and Fig. \ref{fig:diagram_extinguishing} show the previous comment:

%\begin{figure}[t]
%	\centering
%    \includegraphics[scale = 0.6]{images/fire_extinguishing_system.jpeg}
%	\caption{Diagram of the fire extinguishing system installed on ground and aerial platforms.}
%	\label{fig:diagram_extinguishing}
%\end{figure}

%\begin{figure}[t]
%	\centering
%    \includegraphics[scale = 0.6]{images/fire_extinguishing_system_drone.jpg}
%	\caption{Diagram of the fire extinguishing system installed on ground and aerial platforms.}
%	\label{fig:diagram_extinguishing_drone}
%\end{figure}


%For the aerial and ground robot, the arduino board is configured to use mainly the library to communicate with ros (SoftwareSerial.h), this one also allows reading topics and messages of type ROS.  

%In addition, in the ground robot, arduino use a librery to communicate with the servomotors (HerkulexServo.h) that check and read the status of these. 

The fire extinguishing system consists of a set of water pumps that can be activated and deactivated through ROS messages (see Fig. \ref{fig:extinguishing_siar_drone}). 
In the case of the ground robot, the extinguishing device can be aimed by using a pan and tilt unit. When a fire extinguishing task is called, a surveying motion is carried out, and the fire is locked using visual servoing from the measurements from the infrared camera if the fire is confirmed. In the case of the UAVs, the device is fixed, and the UAV frame is used to aim it towards the fire, by controlling only the yaw angle in the inside fires, or motions parallel to the wall for the fires in the facade.

For the fire blankets, given the estimated position of the fire, a trajectory is planned over the fire to release the blanket from the UAV, after checking the actual presence of fire.

%The servomotors are the central part of the 2 DOF robotic arm, where the thermal camera is placed. Thus, we control where to move the thermal camera in tilt and pan position through messages generated by ROS. These messages are sent to the arduino board and this one through its digital pins sends PWM signals to move the servo motors. The motor send back to the arduino a status signal with their position (control closed loop).

%Then, when the thermal camera detect a fire, the pixel fire is centered in the image and arduino activate the water pumps. For this, the arduino sends use the digital pin to send a control signal to the MOSFET switching module and to activate the water pumps. In opposite case the water pumps will stay off.


\subsection{Executive layer}\label{sec:bt}

We employ Behaviour Trees (BTs) as the framework for task execution and monitoring for the robots of the team. BTs are a way to structure the flow and control of multiple tasks in the context of decision-making applications. They are usually presented as an alternative to FSM. First originated as a tool for NPC AI development in the video game industry, BTs have become widespread in robotics, mainly due to its modularity and simplicity \cite{TRO17Colledanchise,paxton2017}.

\begin{figure}[t]
	\centering
    \includegraphics[width = 0.9\textwidth]{images/bt-fireexploration}
	\caption{A simplified BT for a fire exploration mission of a single robot (there are aspects -like fail-safe checks on time and batteries- removed for the sake of clarity). The robot executes an exploration path while looking for a fire. If the fire detection is successful, the robot will approach the fire and command an extinguishing task. Regardless of the result, the robot will go back to the home position.}
	\label{fig:bt-fireexploration}
\end{figure}

While a full description of the BT framework is out of the scope of this paper, here we summarize its main elements. BT model behaviors as hierarchical trees made up of nodes (an example can be seen in Fig. \ref{fig:bt-fireexploration}). Trees are traversed from top to bottom at a given rate following a set of well-defined rules and executing the tasks/commands that are encountered while doing so. Tasks and commands statuses are reported back up in the chain and the flow changes accordingly. A status can be either success, failure or running. According to their functionality, nodes can be classified as:

\begin{itemize}
\item \textbf{Composite}: control the flow through the tree itself and are similar to control structures in traditional programming languages. 
\item \textbf{Decorator}: process or modify the status it receives from its child. 
\item \textbf{Leaf}: this is where the actual task is performed, the atomic tasks that the robot can carry out, or other functionalities. As such, these nodes cannot have any children.
\end{itemize}

As it can be seen from the classification above, BT decouple logic from actual tasks in a natural way. When developing a tree one only should care about the leaf nodes. The flow can later be defined and re-arranged constantly, creating new behaviors and expanding on what is already done. One important benefit of BTs are their composability (due to the hierarchical nature of the trees) and re-usability.

The behavior of the individual robots of the team are created using BTs. In the current case, the leaves are the associated atomic tasks of navigation, fire detection and fire extinguishing as described above, and are integrated using the actionlib interface of ROS. Fig. \ref{fig:bt-fireexploration} presents an example of the behaviour of one robot. We have used a publicly available BT implementation\footnote{\url{https://github.com/BehaviorTree}}, that we have extended to consider the actions and particularities of the application.




\subsection{Cooperation and Coordination}

The approach to Challenge 3 takes advantage of the use of a heterogeneous robot team (mixing UGV and different types of UAVs) for the coordination of the fleet.

On the one hand, each robot specializes on one of the tasks for the Challenge. This means that we consider a loose cooperation between the robots. In particular, we devote the ground robot for the ground floor indoor fire, and each UAV to a different floor (with one UAV for the outside fires and the ground floor fire on the facade). 

Thus, the main aspect to consider is the coordination in time and space to avoid collisions. The task allocation mitigates the risks, as the different vehicles will fly at different heights. In any case, it is important to avoid close encounters between the vehicles.  For that, a priority level is assigned to the different UAVs, and the different facades are visited by each vehicle at different time instants, so that at every moment there no UAV overflying another one. Before proceeding to a new facade, each vehicle checks if a higher priority vehicle is still there. 

Regarding the software architecture, we employ ROS, with different ROS master nodes that run onboard each robot. We use the software described in \cite{pound19} to share between robots only vital information through the wireless network, including the position of each robot for the checks indicated above.







